Talk, Don't Write: A Study of Direct Speech-Based Image Retrieval

Speech-based image retrieval has been studied as a proxy for joint representation learning, usually without emphasis on retrieval itself. As such, it is unclear how well speech-based retrieval can work in practice -- both in an absolute sense and versus alternative strategies that combine automatic speech recognition (ASR) with strong text encoders. In this work, we extensively study and expand choices of encoder architectures, training methodology (including unimodal and multimodal pretraining), and other factors. Our experiments cover different types of speech in three datasets: Flickr Audio, Places Audio, and Localized Narratives. Our best model configuration achieves large gains over state of the art, e.g., pushing recall-at-one from 21.8% to 33.2% for Flickr Audio and 27.6% to 53.4% for Places Audio. We also show our best speech-based models can match or exceed cascaded ASR-to-text encoding when speech is spontaneous, accented, or otherwise hard to automatically transcribe.

==> 30_experimental_setting.tex <==
\section{Experimental Settings}

\paragraph{Speech Preprocessing}{We pad or crop all audio utterances to 40 seconds in {\loca}, 20 seconds for {\places}, 8 seconds for {\flickr}, and 8 seconds for {\conceptual}. Experiments show that those are the optimal length values. We use a publicly available {\cpc} model\cite{kawakami2019unsupervised}\footnote{\cpc authors are in the process of releasing this to the public via tf-hub.} model to extract speech representations in an offline preprocessing step. This model accepts a fixed 20s window of audio as input; longer utterances (in {\loca}) are processed as independent 20 second chunks. The output of {\cpc} is a 1024-d vector representation of each 10ms of audio. (This, notably, is the same frame rate as MFCC frontends in most prior work, and is common in speech processing applications.}


\paragraph{Image Preprocessing}{At training time, images are augmented by randomly brightening and saturating them, and taking a random crop containing $>=67\%$ of the original area. Crops are rescaled to the native resolution of the pretrained image encoder, which is 380x380 for EfficientNet-B4. We use the public TensorFlow Hub implementation of EfficientNet (\footnote{https://tfhub.dev/tensorflow/efficientnet/b4/feature-vector/1}), which comes with ImageNet pretrained weights.}

\paragraph{Encoders}{To extract hidden representation from the image modality, we use an EfficientNet~\cite{tan2019efficientnet}\footnote{\url{https://github.com/qubvel/efficientnet}} pretrained on ImageNet. To have a reference of the overall performance we experiment with a more common ResNet152~\cite{he2016deep}, used in previous work~\cite{harwath2018jointlycv}, to quantify EfficientNet contributions. For the audio modality, we use a ResNet-50 encoder. To compare its performance, we reimplement the audio encoder from~\cite{harwath2016unsupervised} to use it as our baseline ({\harcnn}). For each modality, {\milan} use a 2056-dimensional hidden representation.  All our models use the weights of a model that has been trained on {\conceptual} until convergence, unless specified otherwise.}

\paragraph{Optimization}{We optimize our models using Adam with a learning rate of 0.001 and an exponential decay of 0.999 every 1000 training steps, $\beta_1$ = 0.9, $\beta_2$ = 0.999 and $\epsilon = 10^{-8}$. Our models are trained on 32-core slices of Cloud TPU V3 pods, and except where otherwise specified, use a per-replica batch size of $K = 32$. 


Our training setup pools image and caption encodings
from all replicas before computing the loss.
That is, each replica computes speech and image encodings for its local mini-batch and broadcasts them to all others to be used as negative samples. Training with $N$ cores thus allows the loss to be computed over the global batch of $N \cdot K$ examples and $(N \cdot K)^2$ pairs (in our case 1024 examples and $1024^2$ example pairs).
}


==> IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************


